Discourse vs emissions: Analysis of corporate narratives, symbolic practices, and mimicry through LLMs

Climate change has increased demands for transparent and comparable corporate climate disclosures, yet imitation and symbolic reporting often undermine their value. This paper develops a multidimensional framework to assess disclosure maturity among 828 U.S.listed firms using large language models (LLMs) fine-tuned for climate communication. Four classifiers-sentiment, commitment, specificity, and target ambition-extract narrative indicators from sustainability and annual reports, which are linked to firm attributes such as emissions, market capitalization, and sector. Analyses reveal three insights: (1) risk-focused narratives often align with explicit commitments, but quantitative targets (e.g., net-zero pledges) remain decoupled from tone; (2) larger and higher-emitting firms disclose more commitments and actions than peers, though inconsistently with quantitative targets; and (3) widespread similarity in disclosure styles suggests mimetic behavior, reducing differentiation and decision usefulness. These results highlight the value of LLMs for ESG narrative analysis and the need for stronger regulation to connect commitments with verifiable transition strategies.

==> Comments.tex <==
---REVIEW--POINTS TO IMPROVE----
--can you please check the following comments and which one could be done ?

I provide the review of the manuscript in order to publish it in a high quality research journal,

**“Between words and emissions: LLM evidence on corporate climate narratives, symbolic practices, and mimicry.”** 

I focus on what top-tier journals typically expect (clear causal contribution; transparent, validated measurement; convincing identification; careful statistical inference; reproducibility; and polished exposition) and translate that into concrete, actionable revisions. Citations to your paper point to the relevant passages/tables/figures in the PDF you shared.

---

## Executive summary (what works, and what needs to be strengthened)

**Strengths**

* Timely question at the intersection of climate disclosure, institutional theory, and NLP/LLMs.

* Ambitious cross‑section of 828 U.S. firms and systematic use of ClimateBERT classifiers (sentiment, commitment, specificity, target ambition). 

* Useful descriptive landscape of commitment/specificity/targets with clear tabulations (Tables 3–7, 12–17).

**Key upgrades to reach top‑journal standards**

1. **Sharpen the contribution and the causal question.** Move beyond descriptive patterns to a falsifiable, theory‑driven test (e.g., does investor/regulatory pressure causally increase disclosure “maturity,” net of performance?).

2. **Fix measurement and pipeline issues.** Remove potential selection bias from keyword filtering; correct label logic; validate LLM outputs against human‑coded ground truth; justify thresholds with sensitivity analyses. (3.1–3.3, p. 11)

3. **Replace correlation‑only evidence with econometric modeling.** Use multi‑variable regressions (and, if feasible, quasi‑experimental variation) to link narratives to firm attributes and outcomes with proper controls and uncertainty quantification. 

4. **Make “mimicry” a measured, tested construct.** The current argument infers mimicry from weak cross‑sectional differences; top outlets will want direct similarity metrics and inference. (4.1.4, 5.1–5.3)

5. **Resolve internal inconsistencies and errors.** (a) Reversed labeling logic for reduction vs. net zero; (b) KMeans vs. GMM inconsistency; (c) commitment share stated as 70.3\% elsewhere but 86.5\% in Table 3; (d) the “ISAB (2018) materiality” citation is mismatched. (pp. 11, 16–17, 24–26, 45).

6. **Reproducibility and transparency.** Provide code, model versions, sample construction files, and robustness scripts; add a data/methods appendix. (3–4, Appendix);

7. **Polish exposition and style.** Standardize language (remove French table captions), correct typos, unify notation and sector labels, and streamline the narrative.

---

## Major comments and concrete fixes

### 1) Positioning, theory, and testable predictions

***Clarify the central question**: Are you documenting patterns (**descriptive paper**) or testing mechanisms (**explanatory paper**)? Right now the paper mixes both. For top journals, pick one primary aim and state it in the first paragraph of the introduction and again at the end of 1.

***Tighten hypotheses (2.3).** Each H should make a directional, testable prediction and reflect a specific mechanism (voluntary disclosure vs. legitimacy vs. institutional isomorphism). For example:

***H1 (Legitimacy):** Conditional on sector and size, higher Scope 1–
3 emitters will **increase the share of risk framing** and **reduce opportunity framing**.

***H2 (Voluntary):** Better environmental performers (lower emissions intensity/declining emissions trend) will **set more specific, auditable targets**.

***H3 (Mimicry):** Within-sector, within‑size pairwise narrative similarity is **higher** than across-sector/size similarity after controlling for performance.

Each hypothesis should map to a **specific test** you later run.

### 2) Data and sample construction

* **Document the sampling frame.** Which 828 U.S. firms—exchange(s), sector coverage, exclusion rules, missing data handling? Provide a 



***Missingness (4.1.2, Table 8).** You have substantial missing Scope 3 data (EK: 355 NaNs). Be explicit about **which analyses drop to what N**. Consider **multiple imputation** (with sector/size predictors), or present **missingness as information** (are firms without EK unlike others?).

### 3) Measurement: text pipeline and label construction

***Avoid selection via keyword filtering (3.3).** Filtering paragraphs by a climate keyword list risks **selection-on-observables** and can bias tone/commitment measures (firms with different jargon styles are over/under-counted). Two fixes:

1. Run the classifiers on **all paragraphs**, then **keep those with model‑inferred climate relevance** (probability threshold) rather than a static dictionary.

2. As a robustness check, compare results with and without keyword filtering.

***Paragraph vs. token weighting.** Your report‑level aggregation uses **counts of paragraphs** exceeding thresholds. Paragraph lengths vary: re‑aggregate with **token‑weighted** or **probability‑weighted** averaging of model posteriors. (pp. 10–11);

***Threshold choice and sensitivity.** You fix 30\%/40\% cutoffs for several labels. Replace with:

  ***Cross‑validated thresholds** minimizing misclassification error against a **human‑coded gold set** (draw a stratified sample of \~400 paragraphs across sectors/sizes and double‑code).
  * **Sensitivity plots** showing how main results change when thresholds vary ±10–20 p.p.

    ***Label mapping bug (urgent).** On p. 11, the rule says *if only net‑zero exceeds 30\% → label “reduction”; if only reduction exceeds 30\% → label “netzero”*. That appears reversed. Please fix and re‑run all target‑related analyses. (p. 11);

    ***Classifier validation.** Report **accuracy/F1** on a held‑out hand‑labeled set for each classifier in your corpus. Include **confusion matrices**, **class balance**, and **calibration plots**. Without this, editors will treat the measures as latent and noisy.

### 4) Statistical analysis and identification

***Correlations are not enough.** Spearman ρ’s are small (e.g., −0.42, −0.32, 0.25, 0.34) but highly significant due to N≈828 (Figure 1; Table 2, p=0.007 for one pair). Report **CIs**, apply **multiple‑testing adjustments**, and discuss **economic magnitude**. (p. 30);

***Ordinal coding validity.** Treating *risk → risk\_opportunity → neutral → opportunity* as an ordinal scale is conceptually questionable. Consider **polychoric correlations** for ordinal variables, or **Cramér’s V** for categorical associations. Provide robustness using **one‑hot encodings** in regressions. (4.1.1);

***Move to multivariate models.** Estimate models such as:

  ***Logit/Probit**: `Specificity\_i = f(Emissions, ln(MarketCap), Employees, Sector FE, ReportLength, Year FE)`
  
  ***Ordered Logit** for tone categories; **Multinomial Logit** for target type.
  
  * Report **marginal effects** and **partial R²** to convey substantive size.

***Outcomes and economic significance.** Strengthen the paper by linking narrative maturity to **downstream outcomes**: e.g., next‑year emissions change, cost of capital proxies, analyst forecast dispersion, or climate‑related news sentiment. This moves the paper from “what firms say” to “why it matters.”


### 5) Results presentation and internal consistency

***Consistency check.** In 4.3 you state “high prevalence of climate commitments (70.3\%)” while Table 3 shows **86.5\%** (716/828). Fix the text. (pp. 31, 25–26);

***Net‑zero vs. reduction mix.** After fixing the label bug, revisit 4.1.2–4.1.4 and cluster interpretations (e.g., Clusters 1/6/9). (pp. 16–18, 42);

***Figure and table polish.**

  ***Figure 1 (p. 30):** Add CIs on correlations or a table with CIs below; ensure colorbar ranges are consistent across figures.
  ***Tables 16 & 17:** Avoid “nan\%”. Replace with “N=0” rows removed or annotate “no firms in class.” (pp. 40–41);
  ***Language consistency:** Several tables use French headers (e.g., *Nombre de NaN par colonne*; *Consommation cyclique*). Standardize to English. (pp. 33–41)&#x20;
  ***Units and variable names:** Replace `EI/EJ/EK` by **Scope 1/2/3**; document units and binning rules in a **Table A1: Variable Definitions**.

### 6) Interpretation and policy implications

***Qualify the “greenwashing/symbolic” language.** Where you infer symbolism (e.g., firms with net‑zero but no commitments/specificity), temper the language and show **rates, confounders, and robustness**.

***Regulation references.** Align 5.3 with the **actual U.S./global disclosure landscape** for the study year; specify which results speak to **TCFD/SBTi alignment**, transition plan assurance, or sector‑specific guidance. (pp. 27–29);



## Minor comments (text, style, references)

***Typos/wording:** fix “Forth” → **Fourth**, “gloabally” → **globally**, and remove PDF hyphenation artifacts throughout (e.g., “communication,” “enforcement”). (multiple pages);

***Terminology:** use **“workforce size”** or **“employees”** consistently; unify sector names with standard GICS names. (Tables 12–14);

***Reference accuracy:** The **ISAB (2018)** citation is for a Columbia River fisheries board report (p. 45), not a materiality framework. Replace with authoritative sources on materiality (e.g., SASB/ISSB/SEC guidance) and climate‑reporting specificity.&#x20;

***Consistency of methods section:** 3.4 first says **GMM** then 4.1.3 uses **KMeans**—make these consistent and justify. (pp. 11, 16);

***Numbers and shares:** Always report **N** alongside percentages (you often do; keep it universal) and include **95\% CIs** in text for key shares (e.g., 86.5\% commitments). (Table 3);

***Tables layout:** collapse some very granular tables into appendices; keep the main text focused on the 4–6 most decision‑useful exhibits.

---

## Proposed restructuring

1. **Introduction (2–3 pages)**: Problem → gap → contribution → preview of identification/tests → key results in plain English.

2. **Literature & Hypotheses**: Organize by mechanism; each ends with an explicit testable H.

3. **Data**: Sample frame; sources; missingness; variable definitions table.

4. **Methods**:

   * LLM pipeline (models, validation, aggregation, thresholds, sensitivity plan).
   * Econometric strategy (models, FEs, standard errors, multiple testing).
   * Clustering/similarity (clear choice and diagnostics).
5. **Results**: Main tests first (regressions), then clustering/similarity as complementary evidence, then descriptive.
6. **Robustness & Validations**.
7. **Discussion & Policy**: Tight, mechanism‑consistent, and cautious.
8. **Conclusion & Limitations**: Short and forward‑looking.
9. **Appendices**: Full tables, additional figures, codebook, and validation details.

---

### Title options

-“**Talking alike, acting differently? LLM evidence on climate disclosure maturity and mimicry**”

-“**From tone to targets: Measuring climate disclosure quality with LLMs**”

---

## Table/figure fixes (by location)

***Figure 1 (p. 30):** Add 95\% CIs or a companion table; annotate N; consistent color scales.;

***Tables 12–14 (pp. 36–38):** Standardize sector names to English and GICS; add Ns; move long sector splits to Appendix.;

***Tables 16–17 (pp. 40–41):** Replace “nan\%” rows with “no observations”; clarify binning cutoffs for scopes.;

***Table 8 (p. 34):** Rename to English and report missingness rates (\% of total).;

---

## Reference corrections

## Language and style

## Reproducibility checklist (what to include in an online appendix)



---


